Distributed Delay and Desynchronization in a Brain Network Model

We consider a neural field model which consists of a network of an arbitrary number of Wilson-Cowan nodes with homeostatic adjustment of the inhibitory coupling strength and time delayed, excitatory coupling. We extend previous work on this model to include distributed time delays with commonly used kernel distributions: delta function, uniform distribution and gamma distribution. Focussing on networks which satisfy a constant row sum condition, we show how each eigenvalue of the connectivity matrix may be related to a Hopf bifurcation and that the eigenvalue determines whether the bifurcation leads to synchronized or desynchronized oscillatory behaviour. We consider two example networks, one with all real eigenvalues (bi-directional ring) and one with some complex eigenvalues (uni-directional ring). In bi-directional rings, the Hopf curves are organized so that only the synchronized Hopf leads to asymptotically stable behaviour. Thus the behaviour in the network is always synchronous. In the uni-directional ring networks, however, intersection points of asynchronous and synchronous Hopf curves may occur resulting in double Hopf bifurcation points. Thus asymptotically stable synchronous and asynchronous limit cycles can occur as well as torus-like solutions which combine synchronous and asynchronous behaviour. Increasing the size of the network or the mean time delay makes these intersection points, and the associated asynchronous behaviour, more likely to occur. Numerical approaches are used to confirm the findings, with Hopf bifurcation curves plotted using Wolfram Mathematica. These insights offer a deeper understanding of the mechanisms underlying desynchronization in large networks of oscillators.

==> comparison_plots.tex <==



\subsection{Zero delay}

Let $r_k=\alpha+i\beta $. Then, the   characteristic equation is 
\begin{equation}\label{charac_eq_ODE_uni}
    \lambda^3+p_2\lambda^2+p_1\lambda+p_0-(\alpha+i\beta)  W^Eq\lambda(\lambda+1)=0. 
\end{equation}
Substituting $\lambda=i \omega$ ($\omega>0$ and $i=\sqrt{-1}$) into the characteristic polynomial \eqref{charac_eq_ODE_uni}  gives 
\begingroup
\allowdisplaybreaks
\begin{subequations}
\begin{align}
   \text{Real part: }&(q\alpha-p_2)\omega^2+q\alpha\omega+p_0=0\label{wk_real_part_uni}\\
   \text{Imaginary part: }&\omega \Big(  (q\alpha-p_1)-q\beta\omega-\omega^2\Big)=0\label{wk_img_part_uni}.
\end{align}
\end{subequations}
\endgroup 
From \eqref{wk_real_part_uni}, we have
\[\omega_{\pm}=\cfrac{q\beta\pm \sqrt{q^2\beta^2-4p_0 q \alpha+4p_0 p_2}}{2(p_2-q\alpha)}\]
Substituting $\omega_{\pm}$ in \eqref{wk_real_part_uni} leads to
\begin{equation}\label{eqn_356_uni}
q\left(\cfrac{q\beta\pm \sqrt{q^2\beta^2-4p_0 q \alpha+4p_0 p_2}}{2(p_2-q\alpha)}-\alpha\right) -
\cfrac{\left(q\beta\pm \sqrt{q^2\beta^2-4p_0 q \alpha+4p_0 p_2}\right)^2}{4(p_2-q\alpha)^2}+p_1=0.
\end{equation}
The Hopf curves are implicitly defined by the equation \eqref{eqn_356_uni}  in the $W^{IE},W^E$ parameter space.

When $\beta=0$, equation \eqref{eqn_356_uni} becomes 
\begin{equation}\label{eqn_356_bi}
q\left(\cfrac{\pm \sqrt{4p_0 p_2-4p_0 q \alpha}}{2(p_2-q\alpha)}-\alpha\right) -
\cfrac{4p_0 p_2-4p_0 q \alpha}{4(p_2-q\alpha)^2}+p_1=0.
\end{equation}
\bigskip
When $\alpha=1$, equation \eqref{eqn_356_bi} becomes 
\begin{equation}\label{eqn_356_rk_1}
q\left(\cfrac{\pm \sqrt{4p_0 p_2-4p_0 q}}{2(p_2-q)}-1\right) -
\cfrac{4p_0 p_2-4p_0 q }{4(p_2-q)^2}+p_1=0.
\end{equation}
The plot of equations \ref{eqn_356_uni}-\ref{eqn_356_rk_1} and their approximation are given in Figure \ref{Fig_comparison_plots}.




\subsection{Weak gamma distribution}

Rewrite the characteristic equation \eqref{gammaeq3} as
\begin{equation}\label{charac_weak_kernel_new}
   \Delta_1(\lambda):=\lambda^4+a_3 \lambda^3 
   +\big(a_{22}-r_k a_{23}\big) \lambda^2
   + \big(a_{12}-r_k a_{13}\big) \lambda+a_0=0
\end{equation}
where
\begingroup
\allowdisplaybreaks
\begin{align}\label{coeff_weak_kernel_new}
 a_{22}&=\gamma+\cfrac{1+\gamma}{\tau_1}+\cfrac{K_1  {I^*}^2}{\tau_1\tau_2}-
\cfrac{K_1K_2 \phi^{-1}(p)}{\tau_1 \phi(W^{IE}p)}+\cfrac{W^E K_1K_2 p}{\tau_1 \phi(W^{IE}p)},\qquad 
a_{23}=\cfrac{K_1 W^E \gamma}{\tau_1},\\
 a_{12}&=\cfrac{\gamma}{\tau_1}+\cfrac{K_1 (1+\gamma) {I^*}^2}{\tau_1\tau_2}-
\cfrac{K_1K_2 \gamma \phi^{-1}(p)}{\tau_1 \phi(W^{IE}p)}+\cfrac{W^E K_1K_2 p\gamma}{\tau_1 \phi(W^{IE}p)},\qquad
a_{13}=\cfrac{W^E K_1 \gamma}{\tau_1}. \nonumber
\end{align}
\endgroup
Substituting $\lambda=i \omega$ ($\omega>0$ and $i=\sqrt{-1}$) into the characteristic polynomial \eqref{charac_weak_kernel_new}  yields the following:
\begingroup
\allowdisplaybreaks
\begin{subequations}
\begin{align}
   \text{Real part: }&\omega^{4}+\left(\alpha a_{23}  -a_{22}\right) \omega^{2}+\beta \omega  a_{13}  +a_{0}=0\label{wk_real_part_uni_gamma}\\
   \text{Imaginary part: }&\omega \Big(  \beta \omega  a_{23} -a_{3} \omega^{2}-\alpha  a_{13}+a_{12} \Big)=0\label{wk_img_part_uni_gamma}.
\end{align}
\end{subequations}
\endgroup 
From \eqref{wk_img_part_uni_gamma}, we have
\[\omega_{\pm}=\cfrac{\beta  a_{23}\pm \sqrt{\beta^{2} a_{23}^{2}-4 \alpha  a_{3} a_{13}+4 a_{3} a_{12}}}{2 a_{3}}\]
Substituting $\omega_{\pm}$ in \eqref{wk_real_part_uni_gamma} leads to
\begin{align}
    \label{eqn_356_uni_gamma}
~&\frac{\left(a_{23} \beta +\sqrt{a_{23}^{2} \beta^{2}-4 \alpha  a_{3} a_{13}+4 a_{3} a_{12}}\right)^{4}}{16 a_{3}^{4}}
+\frac{\left(a_{23} \alpha -a_{22}\right) \left(a_{23} \beta +\sqrt{a_{23}^{2} \beta^{2}-4 \alpha  a_{3} a_{13}+4 a_{3} a_{12}}\right)^{2}}{4 a_{3}^{2}}\nonumber\\
~&\hspace{5cm}+\frac{\left(a_{23} \beta \pm\sqrt{a_{23}^{2} \beta^{2}-4 \alpha  a_{3} a_{13}+4 a_{3} a_{12}}\right) a_{13} \beta}{2 a_{3}}+a_{0}=0
\end{align}
The Hopf curves are implicitly defined by the equation \eqref{eqn_356_uni_gamma}  in the $W^{IE},W^E$ parameter space.


When $\beta=0$, equation \eqref{eqn_356_uni_gamma} becomes 
\begin{equation}\label{eqn_356_bi_gamma}
\frac{\left(\alpha a_{13}  -a_{12}\right)^{2}}{a_{3}^{2}}-\frac{\left( \alpha a_{23}-a_{22}\right) \left( \alpha a_{13}-a_{12}\right)}{a_{3}}+a_{0}=0
\end{equation}
\bigskip
When $\alpha=1$, equation \eqref{eqn_356_bi_gamma} becomes 
\begin{equation}\label{eqn_356_rk_1_gamma}
\frac{\left(a_{12}-a_{13}\right)^{2}}{a_{3}^{2}}-\frac{\left(a_{22}-a_{23}\right) \left(a_{12}-a_{13}\right)}{a_{3}}+a_{0}=0
\end{equation}
The plot of equations \ref{eqn_356_uni_gamma}-\ref{eqn_356_rk_1_gamma} and their approximation are given in Figure \ref{Fig_comparison_plots}.

\begin{figure}[H]
     \centering
   \includegraphics[width=1\textwidth]{Figures/Fig_comparison_plots.png}
      \caption{Solid curves are exact, and dashed curves are numerical results.}
      \label{Fig_comparison_plots}
\end{figure}
